CatCMA : Stochastic Optimization for Mixed-Category Problems

Black-box optimization problems often require simultaneously optimizing different types of variables, such as continuous, integer, and categorical variables. Unlike integer variables, categorical variables do not necessarily have a meaningful order, and the discretization approach of continuous variables does not work well. Although several Bayesian optimization methods can deal with mixed-category black-box optimization (MC-BBO), they suffer from a lack of scalability to high-dimensional problems and internal computational cost. This paper proposes CatCMA, a stochastic optimization method for MC-BBO problems, which employs the joint probability distribution of multivariate Gaussian and categorical distributions as the search distribution. CatCMA updates the parameters of the joint probability distribution in the natural gradient direction. CatCMA also incorporates the acceleration techniques used in the covariance matrix adaptation evolution strategy (CMA-ES) and the stochastic natural gradient method, such as step-size adaptation and learning rate adaptation. In addition, we restrict the ranges of the categorical distribution parameters by margin to prevent premature convergence and analytically derive a promising margin setting. Numerical experiments show that the performance of CatCMA is superior and more robust to problem dimensions compared to state-of-the-art Bayesian optimization algorithms.

==> body/old/02_related.tex <==
% ========================================
\section{Related Algorithms} \label{sec:related}
% ========================================


% ------------------------------------
\subsection{CMA-ES}
% ------------------------------------
Covariance matrix adaptation evolution strategy (CMA-ES) is a countinuous black-box optimization algorithm.
The CMA-ES generates candidate solutions in each iteration from the multivariate normal distribution, evaluates the solutions on the objective function, and updates the distribution parameter based on the ranking of the solutions. We introduce a variant of CMA-ES, $(\mu/\muw, \lambda)$-CMA-ES, minimizing $f:\R^N \to \R$.

In the $t$-th iteration, the $\lambda$ candidate solutions $\x_i$ ($i=1, 
\ldots,\lambda$) are generated from the multivariate Gaussian distribution $\mathcal{N}$ as
\begin{align}
    \y_i &\sim \mathcal{N}(\boldsymbol{0}, \C[t]) \enspace, \\
    \x_i &= \m[t] + \sig[t] \y_i \enspace.
\end{align}
The candidate solutions are evaluated on the objective function. We denote that $i:\lambda$ represents the index of $i$-th best sample.

The mean vector $\m[t]$ is updated as
\begin{align}
    \m[t+1] = \m[t] + c_m \sum_{i=1}^{\lambda} w_{i} ( \x_{i:\lambda} - \m[t] ) \enspace,
\end{align}
where $c_m$ is the learning rate for the mean vector, and $w_i$ is the weight that holds $\sum_{i=1}^{\mu} \w_i = 1, \w_1 \geq \w_2 \geq \cdots \geq \w_{\mu} > 0$, $w_{j} = 0\ (j = \mu+1, \ldots,\lambda)$.

The CMA-ES employs the two evolution paths  to cumulate the update direction of the distribution parameter.
\begin{align}
    \ps[t+1] &= (1-c_\sigma)\ps[t] + \sqrt{c_\sigma(2-c_\sigma)\muw} {\C[t]}^{-\frac12} \sum_{i=1}^\lambda \w_i \y_{i:\lambda} \enspace, \\
    \pc[t+1] &= (1-c_c) \pc[t] + h_\sigma \sqrt{c_c(2-c_c)\muw} \sum_{i=1}^\lambda \w_i \y_{i:\lambda} \enspace,
\end{align}
where $\muw = 1 / \sum_{i=1}^{\mu} \w_i^2$, $c_\sigma$ and $c_c$ are cumulative rates, and
\begin{align*}
    h_\sigma \leftarrow \mathds{1} {\left\{\|\ps[t+1]\| < \sqrt{1-(1-c_\sigma)^{2(t+1)}}\left(1.4+\frac{2}{N+1}\right)\E [\|\mathcal{N}(\boldsymbol{0}, \boldsymbol{I}) \|]\right\}}
\end{align*}
is the indicator function to prevent evolutionary path $\pc[t]$ from rapidly lengthening. The expected norm $\E [\|\mathcal{N}(\boldsymbol{0}, \boldsymbol{I}) \|]$ is approximated by $\sqrt{N} \left( 1 - \frac{1}{4 N} + \frac{1}{21 N^2} \right)$.

The covariance matrix $\C[t]$ is updated as
\begin{align}
     &\C[t+1] \leftarrow \left(1 + (1-h_\sigma)c_1 c_c(2-c_c) \right) \C[t] \\
    &+ c_1 \left(\pc[t+1]{\pc[t+1]}^\top - \C[t] \right) + c_\mu \sum_{i=1}^{\lambda} w_i \left( \y_{i:\lambda}\y_{i:\lambda}^\top - \C[t] \right) \enspace,
\end{align}
where $c_1$ and $c_{\mu}$ are the learning rates for the rank-one update and the rank-$\mu$ update, respectively.

The step-size $\sig[t]$ is updated as
\begin{align}
    \sig[t+1] \leftarrow \sig[t] \exp \left( \frac{c_\sigma}{d_\sigma} \left( \frac{\|\ps[t+1] \|}{\E [\|\mathcal{N}(\boldsymbol{0}, \boldsymbol{I}) \|]} - 1 \right) \right) \enspace,
\end{align}
where $d_\sigma$ is a damping factor.

% ------------------------------------
\subsection{Information Geometric Optimization}
% ------------------------------------
The information geometric optimization (IGO)~\cite{IGO:2017} is a unified framework of probabilistic model-based black-box algorithms.
Let $\{P_{\btheta}\}$ be a family of probability distributions on a search space~$\mathcal{X}$ parameterized by $\btheta \in \Theta$.
The IGO transforms the original problem into the maximization of the expected value of $J_{\param[t]} : \Theta \to \R$. The function $J_{\param[t]}$ depends on the current distribution parameter $\param[t]$ and defined as
\begin{align}
    J_{\param[t]} (\btheta) = \int_{\x \in \mathcal{X}} W_{\param[t]}^f (\x) p_{\btheta} (\x) \diff \x \enspace, \label{eq:igo_argmax}
\end{align}
where $W_{\param[t]}^f (\x)$ is the utility function and $p_{\btheta} (\x)$ is the probability density~(mass) function.
The IGO maximizes \eqref{eq:igo_argmax} by natural gradient ascent. The natural gradient $\ngr_\theta J_{\param[t]} (\btheta)$, which is defined by the product of the inverse of Fisher information matrix $F^{-1}(\btheta)$ and the vanilla gradient of $J_{\param[t]} (\btheta)$, is given as
\begin{align}
    \ngr_{\btheta} J_{\param[t]} (\btheta) = \int_{\x \in \mathcal{X}} W_{\param[t]}^f (\x) \ngr_{\btheta} \left( \ln p_{\btheta} (\x) \right) p_{\btheta} (\x)  \diff \x \enspace. \label{eq:IGO-ngr}
\end{align}
The IGO approximates the natural gradient $\ngr_\theta J_{\param[t]} (\btheta)$ at $\btheta = \param[t]$ by the Monte Carlo estimation using $\lambda$ samples $\x_1, \ldots, \x_\lambda$ generated from $P_{\param[t]}$ as
\begin{align}
    \left. \ngr_{\btheta} J_{\param[t]} (\btheta) \right|_{\btheta = \btheta^{(t)}} \approx \frac{1}{\lambda} \sum_{i=1}^\lambda \hat{w}_i \left. \ngr_{\btheta} \ln p_{\btheta} (\x_i) \right|_{\btheta = \param[t]} \enspace,
\end{align}
where $\hat{w}$ is the estimated weight of $W_{\param[t]}^f (\x)$ based on the ranking of the samples. The update rule of the IGO is given as
\begin{align}
    \param[t+1] = \param[t] + \eta  \sum_{i=1}^\lambda \frac{\hat{w}_i}{\lambda} \left. \ngr_{\btheta} \ln p_{\btheta} (\x_i) \right|_{\btheta = {\param[t]}} \enspace,
\end{align}
where $\eta \in \R_{>0}$ is the learning rate.
When the multivariate Gaussian distribution is applied to the IGO framework, we obtain the pure rank-$\mu$ update CMA-ES.


% ------------------------------------
\subsection{Adaptive Stochastic Natural Gradient Method}
% ------------------------------------
+margin correction
